Throughput analysis of RIS-assisted UAV wireless systems under disorientation and misalignment

Reconfigurable intelligent surface (RIS)-assisted unmanned areal vehicles (UAV) communications have been identified as a key enabler of a number of next-generation applications. However, to the best of our knowledge, there is no generalized framework for the quantification of the throughput performance of RIS-assisted UAV systems. Motivated by this, in this paper, we present a comprehensive system model that accounts for the impact of multipath fading, which is modeled by means of mixture gamma, transceiver hardware imperfections, and stochastic beam disorientation and misalignment in order to examine the throughput performance of a RIS-assisted UAV wireless system. In this direction, we present a novel closed-form expression for the system's throughput for two scenarios: i) in the presence and ii) in the absence of disorientation and misalignment. Interestingly, our results reveal the importance of accurate modeling of the aforementioned phenomena as well as the existence of an optimal transmission spectral efficiency.

==> images/organization.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,799); %set diagram left start at 0, and has height of 799
	
	%Straight Lines [id:da7549665141364654] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (50,21) -- (50,760) ;
	%Straight Lines [id:da47625167392970713] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (49,21) -- (86,21) ;
	\draw [shift={(89,21)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da14186589472175903] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,111) -- (88,111) ;
	\draw [shift={(91,111)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9483543763704907] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,140) -- (88,140) ;
	\draw [shift={(91,140)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da7917046674146371] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,170) -- (88,170) ;
	\draw [shift={(91,170)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da49631263983654694] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,200) -- (108,200) ;
	\draw [shift={(111,200)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da704360701576451] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,170) -- (71,381) ;
	%Straight Lines [id:da45229232300561106] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,229) -- (128,229) ;
	\draw [shift={(131,229)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da03584291262622097] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,200) -- (91,350) ;
	%Straight Lines [id:da616440142730736] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (92,260) -- (129,260) ;
	\draw [shift={(132,260)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da11951286587293786] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,260) -- (112,321) ;
	%Straight Lines [id:da27642545962354803] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,291) -- (149,291) ;
	\draw [shift={(152,291)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da5459855164810739] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,321) -- (149,321) ;
	\draw [shift={(152,321)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da5348702022757221] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,350) -- (127,350) ;
	\draw [shift={(130,350)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9867014456859513] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,381) -- (108,381) ;
	\draw [shift={(111,381)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6418925655118273] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,409) -- (128,409) ;
	\draw [shift={(131,409)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9876986683837687] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,380) -- (91,530) ;
	%Straight Lines [id:da8287168204190516] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (92,440) -- (129,440) ;
	\draw [shift={(132,440)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9576983292731358] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,440) -- (112,501) ;
	%Straight Lines [id:da6803705166706564] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,471) -- (149,471) ;
	\draw [shift={(152,471)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da3190777351415839] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,501) -- (149,501) ;
	\draw [shift={(152,501)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da04645716603992289] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,530) -- (127,530) ;
	\draw [shift={(130,530)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da999392842419778] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (50,561) -- (87,561) ;
	\draw [shift={(90,561)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da04270397591269859] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,583) -- (107,583) ;
	\draw [shift={(110,583)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da13839239630828648] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,612) -- (127,612) ;
	\draw [shift={(130,612)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9486747809556244] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,583) -- (90,643) ;
	%Straight Lines [id:da36389262070872097] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,643) -- (127,643) ;
	\draw [shift={(130,643)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da7501450490403929] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,561) -- (70,670) ;
	%Straight Lines [id:da11114295170924793] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,670) -- (107,670) ;
	\draw [shift={(110,670)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da35497592028348324] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,699) -- (127,699) ;
	\draw [shift={(130,699)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6435599189355405] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,670) -- (90,730) ;
	%Straight Lines [id:da0883718619590077] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,730) -- (127,730) ;
	\draw [shift={(130,730)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6124523428698243] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (50,760) -- (87,760) ;
	\draw [shift={(90,760)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da8997117662877758] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,21) -- (71,81) ;
	%Straight Lines [id:da8859923266700584] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,50) -- (108,50) ;
	\draw [shift={(111,50)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6960125977451803] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,81) -- (108,81) ;
	\draw [shift={(111,81)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	
	% Text Node
	\draw (167.04,19.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I - Introduction}};
	% Text Node
	\draw (177.04,109.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. II - System model}};
	% Text Node
	\draw (261.04,139.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. III - E2e channel statistical characterization}};
	% Text Node
	\draw (204.04,169.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV - Performance analysis}};
	% Text Node
	\draw (222.04,199.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV-A - Ideal RF front-end}};
	% Text Node
	\draw (249.04,228.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A1 - Instantaneous SNR}};
	% Text Node
	\draw (195.04,259.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - OP}};
	% Text Node
	\draw (296.04,289.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {Without disorientation and misalignment};
	% Text Node
	\draw (286.04,319.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {With disorientation and misalignment};
	% Text Node
	\draw (232.04,349.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A3 - Diversity order}};
	% Text Node
	\draw (238.04,379.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV-B - Non-ideal RF front-end}};
	% Text Node
	\draw (255.04,408.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - Instantaneous SDNR}};
	% Text Node
	\draw (195.04,439.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - OP}};
	% Text Node
	\draw (296.04,469.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {Without disorientation and misalignment};
	% Text Node
	\draw (286.04,499.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {With disorientation and misalignment};
	% Text Node
	\draw (232.04,529.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A3 - Diversity order}};
	% Text Node
	\draw (199.04,558.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V - Results \& discussion}};
	% Text Node
	\draw (220.04,582.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V-A - Ideal RF front-end}};
	% Text Node
	\draw (315.04,613) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-A1 - }Without disorientation and misalignment};
	% Text Node
	\draw (305.04,643) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-A2 - With} disorientation and misalignment};
	% Text Node
	\draw (236.04,671.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V-B - Non-ideal RF front-end}};
	% Text Node
	\draw (315.04,700) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-B1 - }Without disorientation and misalignment};
	% Text Node
	\draw (305.04,730) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-B2 - With} disorientation and misalignment};
	% Text Node
	\draw (173.04,761.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. VI - Conclusions}};
	% Text Node
	\draw (237.04,49.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I-A - Novelty and contribution}};
	% Text Node
	\draw (247.04,80.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I-B - Organization and notations}};
	
	
\end{tikzpicture}

